Doubly Random Parallel Stochastic Methods for Large Scale Learning

We consider learning problems over training sets in which both, the number of training examples and the dimension of the feature vectors, are large. To solve these problems we propose the random parallel stochastic algorithm (RAPSA). We call the algorithm random parallel because it utilizes multiple processors to operate in a randomly chosen subset of blocks of the feature vector. We call the algorithm parallel stochastic because processors choose elements of the training set randomly and independently. Algorithms that are parallel in either of these dimensions exist, but RAPSA is the first attempt at a methodology that is parallel in both, the selection of blocks and the selection of elements of the training set. In RAPSA, processors utilize the randomly chosen functions to compute the stochastic gradient component associated with a randomly chosen block. The technical contribution of this paper is to show that this minimally coordinated algorithm converges to the optimal classifier when the training objective is convex. In particular, we show that: (i) When using decreasing stepsizes, RAPSA converges almost surely over the random choice of blocks and functions. (ii) When using constant stepsizes, convergence is to a neighborhood of optimality with a rate that is linear in expectation. RAPSA is numerically evaluated on the MNIST digit recognition problem.

==> ARAPSA.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%    S   E   C   T   I   O   N    %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Accelerated Random Parallel Stochastic Algorithm (ARAPSA)}\label{sec:arapsa}

As we mentioned in Section \ref{sec:rapsa}, RAPSA operates on first-order information which may lead to slow convergence in ill-conditioned problems. We introduce Accelerated RAPSA (ARAPSA) as a parallel doubly stochastic algorithm that incorporates second-order information of the objective by separately approximating the function curvature for different blocks. We do this by implementing the oLBFGS algorithm for different blocks of the variable $\bbx$. Define $\hbB_i^t$ as an approximation for the Hessian inverse of the objective function that corresponds to the block $\bbx_i$. The update of ARAPSA is defined as multiplication of the descent direction of RAPSA by $\hbB_i^t$, i.e. 
%%
\begin{equation}\label{ARAPS_update}
\bbx^{t+1}_{i}  \ = \ \bbx^{t}_{i}  - \gamma^t\  \hbB_i^t\ \nabla_{\bbx_i} f( \bbx^{t}, \bbTheta_i^t) \qquad \forall \ \bbx_i\in \ccalS^t.
\end{equation}
%%
We next detail how to properly specify the block approximate Hessian $\hbB_i^t$  so that it behaves in a manner comparable to the true Hessian. To do so, define for each block coordinate $\bbx_i$ at step $t$ the variable variation $\bbv_i^t$ and the stochastic gradient variation $\hbr_i^t$ as
%%
%%
\begin{equation}\label{var_grad_var}
\bbv_i^t \:=\ \bbx^{t+1}_{i}  - \bbx^{t}_{i} , \qquad 
\hbr_i^t \:=\ \nabla_{\bbx_i} f( \bbx^{t+1}, \bbTheta_i^t)  - \nabla_{\bbx_i} f( \bbx^{t}, \bbTheta_i^t).
\end{equation}
%%
Observe that the stochastic gradient variation $\hbr_i^t$ is defined as the difference of stochastic gradients at times $t+1$ and $t$ corresponding to the block $\bbx_i$ for a common set of realizations $\bbTheta_i^t$. The term $ \nabla_{\bbx_i} f( \bbx^{t}, \bbTheta_i^t)$ is the same as the stochastic gradient used at time $t$ in \eqref{ARAPS_update}, while $\nabla_{\bbx_i} f( \bbx^{t+1}, \bbTheta_i^t)$ is computed only to determine the stochastic gradient variation $\hbr_i^t$. An alternative and perhaps more natural definition for the stochastic gradient variation is $\nabla_{\bbx_i} f( \bbx^{t+1}, \bbTheta_i^{t+1})  - \nabla_{\bbx_i} f( \bbx^{t}, \bbTheta_i^t)$. However, as pointed out in \cite{schraudolph2007stochastic}, this formulation is insufficient for establishing the convergence of stochastic quasi-Newton methods. We proceed to developing a block-coordinate quasi-Newton method by first noting an important property of the true Hessian, and design our approximate scheme to satisfy this property. In particular, observe that the true Hessian inverse $(\bbH_i^t)^{-1}$ corresponding to block $\bbx_i$ satisfies the block secant condition, stated as $
(\bbH_i^t)^{-1}\bbv_i^{t}=\hbr_i^{t}
$ 
 when the iterates $\bbx_i^t$ and $\bbx_i^{t+1}$ are close to each other. The secant condition may be interpreted as stating that the stochastic gradient of a quadratic approximation of the objective function evaluated at the next iteration agrees with the stochastic gradient at the current iteration. We select a Hessian inverse approximation matrix associated with block $\bbx_i$ such that it satisfies the secant condition $\hbB_i^{t+1}\bbv_i^{t}=\hbr_i^{t}$, and thus behaves in a comparable manner to the true block Hessian. 
 
 The oLBFGS Hessian inverse update rule maintains the secant condition at each iteration by using information of the last $\tau\geq1$ pairs of variable and stochastic gradient variations $\{\bbv_i^u,\hbr_i^{u}\}_{u=t-\tau}^{t-1}$. To state the update rule of oLBFGS for revising the Hessian inverse approximation matrices of the blocks, define a matrix as $\hbB_i^{t,0}:= \eta_i^t\bbI$ for each block $i$ and $t$, where the constant $\eta_i^t$ for $t>0$ is given by
%%
\begin{equation}\label{initial_matrix_update}
\eta_i^t:= \frac{(\bbv_i^{t-1})^{T}\hbr_i^{t-1}}{\|\hbr_i^{t-1}\|^2},
\end{equation}
%%
while the initial value is $\eta_i^t=1$.
The matrix $\hbB_i^{t,0}$ is the initial approximate for the Hessian inverse associated with block $\bbx_i$. The approximate matrix $\hbB_i^{t}$ is computed by updating the initial matrix $\hbB_i^{t,0}$ using the last $\tau $ pairs of curvature information $\{\bbv_i^u,\hbr_i^{u}\}_{u=t-\tau}^{t-1}$. We define the approximate Hessian inverse $\hbB_i^{t}=\hbB_i^{t,\tau}$ corresponding to block $\bbx_i$ at step $t$ as the outcome of $\tau$ recursive applications of the update
%
\begin{equation}\label{SLBFGS_update}
   \hbB_i^{t,u+1}
      =   (\hbZ_i^{t-\tau+u})^T\ \!
                \hbB_i^{t,u}\ \! (\hbZ_i^{t-\tau+u})   
            + \hat{ \rho}_i^{t-\tau+u} \ \!(\bbv_i^{t-\tau+u})\ \!(\bbv_i^{t-\tau+u})^{T},
\end{equation}
%
where the matrices $\hbZ_i^{t-\tau+u}$ and the constants $\hat{\rho}_i^{t-\tau+u} $ in \eqref{SLBFGS_update} for $u=0,\dots, \tau-1$ are defined as 
%
\begin{equation}\label{Z_rho_definitions}
   \hat{\rho}_i^{t-\tau+u}\ =\ \frac{1}{(\bbv_i^{t-\tau+u})^{T}\hbr_i^{t-\tau+u}}
   \quad \text{and}\quad
   \hbZ_i^{t-\tau+u}\ =\ \bbI - \hat{\rho}_i^{t-\tau+u} \hbr_i^{t-\tau+u} (\bbv_i^{t-\tau+u})^{T}.
\end{equation}
%
The computation cost of $\hbB_i^{t}$ in \eqref{SLBFGS_update} is in the order of $O(p_i^2)$, however, for the update in \eqref{ARAPS_update} the descent direction $\hbd_i^t := \hbB_i^{t} \nabla_{\bbx_i} f( \bbx^{t}, \bbTheta_i^t) $ is required. \cite{DingNocedal} introduces an efficient implementation of product $\hbB_i^{t} \nabla_{\bbx_i} f( \bbx^{t}, \bbTheta_i^t)$ that requires computation complexity of order $O(\tau p_i)$. We use the same idea for computing the descent direction of ARAPSA for each block -- more details are provided in supplementary materials. Therefore, the computation complexity of updating each block for ARAPSA is in the order of  $O(\tau p_i)$, while RAPSA requires $O( p_i)$ operations. 
On the other hand, ARAPSA accelerates the convergence of RAPSA by incorporating the second order information of the objective function for the block updates, as may be observed in the numerical analyses provided in Section \ref{sec:simulations}. 









==> Rate.tex <==
%!TEX root = root.tex
%\subsection{Rate of Convergence} \label{sec:rate}\vspace{-2mm}
%\red{In this section we investigate the rate of convergence for the regularized stochastic BFGS. In \cite{Dennis,Powell,Byrd, Nocedal} it has been shown that the rate of convergence for deterministic BFGS is super-linear under the condition that the sequence of step sizes is chosen based on some line search algorithms, e.g. Wolfe conditions. In stochastic settings line searches are problematic, since the value of descent function is not available for all the points. As a consequence in stochastic optimization constant or diminishing step sizes are applied which avoids achieving a super-linear rate of convergence. In the following Theorem we show that the rate of convergence for regularized stochastic BFGS in terms of expectation of the objective function error is linear.} \blue{This is just a long excuse for not proving a stronger result. Just say what the theorem claims and that's it.}
We complement the convergence result in Theorem \ref{convg} with a characterization of the expected convergence rate that we introduce in the following theorem.
%
\begin{theorem}\label{theo_convergence_rate}
Consider the online Limited memory BFGS algorithm as defined by \eqref{eqn_olbfgs_descent}-\eqref{initial_matrix_update_2}. If assumptions \ref{ass_intantaneous_hessian_bounds}, \ref{ass_bounded_stochastic_gradient_norm} and \ref{stepsize_ass} hold true and the step size parameters $\eps_0$ and $T_{0}$ satisfy the inequality
%
\begin{equation}\label{eqn_thm_cvg_rate_10}
    2\  \epsilon_{0} T_{0} \delta >1\ ,
\end{equation} 
%
then the optimal objective $F(\bbw^*)$ satisfies 
%
\vspace{-2mm}
\begin{equation}\label{eqn_thm_cvg_rate_20}
\E {F(\bbw_{t})}- F(\bbw^*)\ \leq\ \frac{C_{0}}{T_{0}+t}\ ,\vspace{-2mm}
\end{equation}
%
where the constant $C_{0}$ satisfies
%
\vspace{-2mm}
\begin{equation}\label{eqn_thm_cvg_rate_30}
 C_{0} = \max \left\{ \frac{\epsilon_{0}^{2}\   T_{0}^{2} K}{2 \epsilon_{0} T_{0} \delta -1}, T_{0}\ \!  (F(\bbw_{0}) -\ F(\bbw^*))  \right\} .\vspace{-2mm}
\end{equation}
%
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Proof of Theorem 2
%
%\begin{proof} 
%See Supplementary Material.
 %\end{proof}

Theorem \ref{theo_convergence_rate} shows that under specified assumptions, the expected error  in terms of the objective value after $t$ oLBFGS iterations is of order $O(1/t)$. This implies that the rate of convergence for oLBFGS is not better than conventional SGD. While the convergence rate doesn't change, improvements in convergence time are marked as we illustrate with the numerical experiments of section \ref{sec_ad_numerical_results}.




==> my_sections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\smallskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



\newenvironment{indentedparagraph}[1] 
{\begin{list}{}%
         {\setlength{\leftmargin}{11pt}
          \setlength{\topsep}{10pt}}
         \item[]{\it #1.}}
{\end{list}}


